Identifying RR Lyrae in the ZTF DR3 dataset

We present a RR Lyrae (RRL) catalogue based on the combination of the third data release of the Zwicky Transient Facility (ZTF DR3) and \textit{Gaia} EDR3. We use a multi-step classification pipeline relying on the Fourier decomposition fitting to the multi-band ZTF light curves and random forest classification. The resulting catalogue contains 71,755 RRLs with period and light curve parameter measurements and has completeness of 0.92 and purity of 0.92 with respect to the SOS \textit{Gaia} DR2 RRLs. The catalogue covers the Northern sky with declination $\geq -28^\circ$, its completeness is $\gtrsim 0.8$ for heliocentric distance $\leq 80$~kpc, and the most distant RRL at 132~kpc. Compared with several other RRL catalogues covering the Northern sky, our catalogue has more RRLs around the Galactic halo and is more complete at low Galactic latitude areas. Analysing the spatial distribution of RRL in the catalogue reveals the previously known major over-densities of the Galactic halo, such as the Virgo over-density and the Hercules-Aquila Cloud, with some evidence of an association between the two. We also analyse the Oosterhoff fraction differences throughout the halo, comparing it with the density distribution, finding increasing Oosterhoff I fraction at the elliptical radii between 16 and 32 kpc and some evidence of different Oosterhoff fractions across various halo substructures.

==> bib.tex <==
@dataset{huang_kuan_wei_2021_5774018,
  author       = {Huang, Kuan-Wei and
                  Koposov, Sergey E.},
  title        = {The RR Lyrae variable catalog of ZTF DR3},
  month        = dec,
  year         = 2021,
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.5774018},
  url          = {https://doi.org/10.5281/zenodo.5774018}
}



@article{scikit-learn,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}


@ARTICLE{Iorio2021,
       author = {{Iorio}, Giuliano and {Belokurov}, Vasily},
        title = "{Chemo-kinematics of the Gaia RR Lyrae: the halo and the disc}",
      journal = {\mnras},
     keywords = {stars: variables: RR Lyrae, Galaxy: disc, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: stellar content, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {502},
       number = {4},
        pages = {5686-5710},
          doi = {10.1093/mnras/stab005},
archivePrefix = {arXiv},
       eprint = {2008.02280},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502.5686I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@software{sqlutilpy,
  author       = {Sergey Koposov},
  title        = {segasai/sqlutilpy: sqlutilpy v0.16.0},
  month        = aug,
  year         = 2021,
  publisher    = {Zenodo},
  version      = {0.16.0},
  doi          = {10.5281/zenodo.5160119},
  url          = {https://doi.org/10.5281/zenodo.5160119}
}

@ARTICLE{2020MNRAS.498.5574E,
       author = {{Erkal}, Denis and {Belokurov}, Vasily A. and {Parkin}, Daniel L.},
        title = "{Equilibrium models of the Milky Way mass are biased high by the LMC}",
      journal = {\mnras},
     keywords = {Galaxy: evolution, Galaxy: halo, Galaxy: kinematics and dynamics, Magellanic Clouds, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = nov,
       volume = {498},
       number = {4},
        pages = {5574-5580},
          doi = {10.1093/mnras/staa2840},
archivePrefix = {arXiv},
       eprint = {2001.11030},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.498.5574E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{Statistics01randomforests,
    author = {Leo Breiman},
    title = {Random Forests},
    booktitle = {Machine Learning},
    year = {2001},
    pages = {5--32}
}




@ARTICLE{2019ApJ...884...51G,
       author = {{Garavito-Camargo}, Nicolas and {Besla}, Gurtina and {Laporte}, Chervin F.~P. and {Johnston}, Kathryn V. and {G{\'o}mez}, Facundo A. and {Watkins}, Laura L.},
        title = "{Hunting for the Dark Matter Wake Induced by the Large Magellanic Cloud}",
      journal = {\apj},
     keywords = {Galaxy: kinematics and dynamics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2019,
        month = oct,
       volume = {884},
       number = {1},
          eid = {51},
        pages = {51},
          doi = {10.3847/1538-4357/ab32eb},
archivePrefix = {arXiv},
       eprint = {1902.05089},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...884...51G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2021Natur.592..534C,
       author = {{Conroy}, Charlie and {Naidu}, Rohan P. and {Garavito-Camargo}, Nicol{\'a}s and {Besla}, Gurtina and {Zaritsky}, Dennis and {Bonaca}, Ana and {Johnson}, Benjamin D.},
        title = "{All-sky dynamical response of the Galactic halo to the Large Magellanic Cloud}",
      journal = {\nat},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jan,
       volume = {592},
       number = {7855},
        pages = {534-536},
          doi = {10.1038/s41586-021-03385-7},
archivePrefix = {arXiv},
       eprint = {2104.09515},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021Natur.592..534C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{1976Ap&SS..39..447L,
       author = {{Lomb}, N.~R.},
        title = "{Least-Squares Frequency Analysis of Unequally Spaced Data}",
      journal = {\apss},
     keywords = {Astronomy, Data Reduction, Least Squares Method, Background Noise, Power Spectra, Sine Waves, Spectrum Analysis, Statistical Analysis, Variable Stars, Astronomy},
         year = 1976,
        month = feb,
       volume = {39},
       number = {2},
        pages = {447-462},
          doi = {10.1007/BF00648343},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1976Ap&SS..39..447L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{1982ApJ...263..835S,
       author = {{Scargle}, J.~D.},
        title = "{Studies in astronomical time series analysis. II. Statistical aspects of spectral analysis of unevenly spaced data.}",
      journal = {\apj},
     keywords = {Astronomy, Signal Detection, Spectrum Analysis, Statistical Distributions, Time Series Analysis, Fourier Transformation, Frequency Response, Power Spectra, Signal To Noise Ratios, Astronomy},
         year = 1982,
        month = dec,
       volume = {263},
        pages = {835-853},
          doi = {10.1086/160554},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982ApJ...263..835S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2018ApJS..236...16V,
       author = {{VanderPlas}, Jacob T.},
        title = "{Understanding the Lomb-Scargle Periodogram}",
      journal = {\apjs},
     keywords = {methods: data analysis, methods: statistical, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = may,
       volume = {236},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/1538-4365/aab766},
archivePrefix = {arXiv},
       eprint = {1703.09824},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..236...16V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2016ApJ...817...73H,
       author = {{Hernitschek}, Nina and {Schlafly}, Edward F. and {Sesar}, Branimir and {Rix}, Hans-Walter and {Hogg}, David W. and {Ivezi{\'c}}, {\v{Z}}eljko and {Grebel}, Eva K. and {Bell}, Eric F. and {Martin}, Nicolas F. and {Burgett}, W.~S. and {Flewelling}, H. and {Hodapp}, K.~W. and {Kaiser}, N. and {Magnier}, E.~A. and {Metcalfe}, N. and {Wainscoat}, R.~J. and {Waters}, C.},
        title = "{Finding, Characterizing, and Classifying Variable Sources in Multi-epoch Sky Surveys: QSOs and RR Lyrae in PS1 3{\ensuremath{\pi}} data}",
      journal = {\apj},
     keywords = {methods: statistical, quasars: general, stars: variables: RR Lyrae, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = jan,
       volume = {817},
       number = {1},
          eid = {73},
        pages = {73},
          doi = {10.3847/0004-637X/817/1/73},
archivePrefix = {arXiv},
       eprint = {1511.05527},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817...73H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2011ApJ...737..103S,
       author = {{Schlafly}, Edward F. and {Finkbeiner}, Douglas P.},
        title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
      journal = {\apj},
     keywords = {dust, extinction, Galaxy: stellar content, ISM: clouds, Astrophysics - Galaxy Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {2},
          eid = {103},
        pages = {103},
          doi = {10.1088/0004-637X/737/2/103},
archivePrefix = {arXiv},
       eprint = {1012.4804},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737..103S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2014ApJS..213....9D,
       author = {{Drake}, A.~J. and {Graham}, M.~J. and {Djorgovski}, S.~G. and {Catelan}, M. and {Mahabal}, A.~A. and {Torrealba}, G. and {Garc{\'\i}a-{\'A}lvarez}, D. and {Donalek}, C. and {Prieto}, J.~L. and {Williams}, R. and {Larson}, S. and {Christen sen}, E. and {Belokurov}, V. and {Koposov}, S.~E. and {Beshore}, E. and {Boattini}, A. and {Gibbs}, A. and {Hill}, R. and {Kowalski}, R. and {Johnson}, J. and {Shelly}, F.},
        title = "{The Catalina Surveys Periodic Variable Star Catalog}",
      journal = {\apjs},
     keywords = {catalogs, Galaxy: halo, Galaxy: stellar content, Galaxy: structure, techniques: photometric, stars: variables: general, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jul,
       volume = {213},
       number = {1},
          eid = {9},
        pages = {9},
          doi = {10.1088/0067-0049/213/1/9},
archivePrefix = {arXiv},
       eprint = {1405.4290},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..213....9D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2020ApJS..249...18C,
       author = {{Chen}, Xiaodian and {Wang}, Shu and {Deng}, Licai and {de Grijs}, Richard and {Yang}, Ming and {Tian}, Hao},
        title = "{The Zwicky Transient Facility Catalog of Periodic Variable Stars}",
      journal = {\apjs},
     keywords = {Periodic variable stars, Pulsating variable stars, Cepheid variable stars, RR Lyrae variable stars, Delta Scuti variable stars, Long period variable stars, Mira variable stars, Eclipsing binary stars, Galaxy structure, Distance indicators, 1213, 1307, 218, 1410, 370, 935, 1066, 444, 622, 394, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
       volume = {249},
       number = {1},
          eid = {18},
        pages = {18},
          doi = {10.3847/1538-4365/ab9cae},
archivePrefix = {arXiv},
       eprint = {2005.08662},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJS..249...18C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2017AJ....153..204S,
       author = {{Sesar}, Branimir and {Hernitschek}, Nina and {Mitrovi{\'c}}, Sandra and {Ivezi{\'c}}, {\v{Z}}eljko and {Rix}, Hans-Walter and {Cohen}, Judith G. and {Bernard}, Edouard J. and {Grebel}, Eva K. and {Martin}, Nicolas F. and {Schlafly}, Edward F. and {Burgett}, William S. and {Draper}, Peter W. and {Flewelling}, Heather and {Kaiser}, Nick and {Kudritzki}, Rolf P. and {Magnier}, Eugene A. and {Metcalfe}, Nigel and {Tonry}, John L. and {Waters}, Christopher},
        title = "{Machine-learned Identification of RR Lyrae Stars from Sparse, Multi-band Data: The PS1 Sample}",
      journal = {\aj},
     keywords = {catalogs, Galaxy: halo, methods: data analysis, methods: statistical, stars: variables: RR Lyrae, surveys, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = may,
       volume = {153},
       number = {5},
          eid = {204},
        pages = {204},
          doi = {10.3847/1538-3881/aa661b},
archivePrefix = {arXiv},
       eprint = {1611.08596},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....153..204S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2020arXiv201201533G,
       author = {{Gaia Collaboration} and {Brown}, A.~G.~A. and {Vallenari}, A. and {Prusti}, T. and {de Bruijne}, J.~H.~J. and {Babusiaux}, C. and {Biermann}, M.},
        title = "{Gaia Early Data Release 3: Summary of the contents and survey properties}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.01533},
        pages = {arXiv:2012.01533},
archivePrefix = {arXiv},
       eprint = {2012.01533},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201201533G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{Catelan_2004,
	doi = {10.1086/422916},
	url = {https://doi.org/10.1086/422916},
	year = 2004,
	month = {oct},
	publisher = {American Astronomical Society},
	volume = {154},
	number = {2},
	pages = {633--649},
	author = {M. Catelan and Barton J. Pritzl and Horace A. Smith},
	title = {The {RR} Lyrae Period-Luminosity Relation. I. Theoretical Calibration},
	journal = {The Astrophysical Journal Supplement Series}
}



@ARTICLE{2015ApJ...798L..12F,
       author = {{Fiorentino}, Giuliana and {Bono}, Giuseppe and {Monelli}, Matteo and {Stetson}, Peter B. and {Tolstoy}, Eline and {Gallart}, Carme and {Salaris}, Maurizio and {Mart{\'\i}nez-V{\'a}zquez}, Clara E. and {Bernard}, Edouard J.},
        title = "{Weak Galactic Halo-Dwarf Spheroidal Connection from RR Lyrae Stars}",
      journal = {\apjl},
     keywords = {Local Group, stars: variables: RR Lyrae, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jan,
       volume = {798},
       number = {1},
          eid = {L12},
        pages = {L12},
          doi = {10.1088/2041-8205/798/1/L12},
archivePrefix = {arXiv},
       eprint = {1411.7300},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...798L..12F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2014PASP..126..616S,
       author = {{Stetson}, Peter B. and {Fiorentino}, Giuliana and {Bono}, Giuseppe and {Bernard}, Edouard J. and {Monelli}, Matteo and {Iannicola}, Giacinto and {Gallart}, Carme and {Ferraro}, Ivan},
        title = "{Homogeneous Photometry VI: Variable Stars in the Leo I Dwarf Spheroidal Galaxy}",
      journal = {\pasp},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jul,
       volume = {126},
       number = {941},
        pages = {616},
          doi = {10.1086/677352},
archivePrefix = {arXiv},
       eprint = {1406.6704},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014PASP..126..616S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2004AJ....127.1158V,
       author = {{Vivas}, A.~K. and {Zinn}, R. and {Abad}, C. and {Andrews}, P. and {Bailyn}, C. and {Baltay}, C. and {Bongiovanni}, A. and {Brice{\~n}o}, C. and {Bruzual}, G. and {Coppi}, P. and {Della Prugna}, F. and {Ellman}, N. and {Ferr{\'\i}n}, I. and {Gebhard}, M. and {Girard}, T. and {Hernandez}, J. and {Herrera}, D. and {Honeycutt}, R. and {Magris}, G. and {Mufson}, S. and {Musser}, J. and {Naranjo}, O. and {Rabinowitz}, D. and {Rengstorf}, A. and {Rosenzweig}, P. and {S{\'a}nchez}, Ge. and {S{\'a}nchez}, Gu. and {Schaefer}, B. and {Schenner}, H. and {Snyder}, J.~A. and {Sofia}, S. and {Stock}, J. and {van Altena}, W. and {Vicente}, B. and {Vieira}, K.},
        title = "{The QUEST RR Lyrae Survey. I. The First Catalog}",
      journal = {\aj},
     keywords = {Galaxy: Halo, Stars: Variables: Other, Surveys},
         year = 2004,
        month = feb,
       volume = {127},
       number = {2},
        pages = {1158-1175},
          doi = {10.1086/380929},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AJ....127.1158V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{Vivas_2006,
	doi = {10.1086/505200},
	url = {https://doi.org/10.1086/505200},
	year = 2006,
	month = {jun},
	publisher = {American Astronomical Society},
	volume = {132},
	number = {2},
	pages = {714--728},
	author = {A. Katherina Vivas and Robert Zinn},
	title = {The {QUEST} {RR} Lyrae Survey. {II}. The Halo Overdensities in the First Catalog},
	journal = {The Astronomical Journal}
}


@ARTICLE{2015MNRAS.446.2251T,
       author = {{Torrealba}, G. and {Catelan}, M. and {Drake}, A.~J. and {Djorgovski}, S.~G. and {McNaught}, R.~H. and {Belokurov}, V. and {Koposov}, S. and {Graham}, M.~J. and {Mahabal}, A. and {Larson}, S. and {Christensen}, E.},
        title = "{Discovery of {\ensuremath{\sim}}9000 new RR Lyrae in the southern Catalina surveys}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: statistical, stars: variables: RR Lyrae, Galaxy: halo, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2015,
        month = jan,
       volume = {446},
       number = {3},
        pages = {2251-2266},
          doi = {10.1093/mnras/stu2274},
archivePrefix = {arXiv},
       eprint = {1410.7653},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.446.2251T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{10.1093/mnras/stz2609,
    author = {Martínez-Vázquez, C E and Vivas, A K and Gurevich, M and Walker, A R and McCarthy, M and Pace, A B and Stringer, K M and Santiago, B and Hounsell, R and Macri, L and Li, T S and Bechtol, K and Riley, A H and Kim, A G and Simon, J D and Drlica-Wagner, A and Nadler, E O and Marshall, J L and Annis, J and Avila, S and Bertin, E and Brooks, D and Buckley-Geer, E and Burke, D L and Carnero Rosell, A and Carrasco Kind, M and da Costa, L N and De Vicente, J and Desai, S and Diehl, H T and Doel, P and Everett, S and Frieman, J and García-Bellido, J and Gaztanaga, E and Gruen, D and Gruendl, R A and Gschwend, J and Gutierrez, G and Hollowood, D L and Honscheid, K and James, D J and Kuehn, K and Kuropatkin, N and Maia, M A G and Menanteau, F and Miller, C J and Miquel, R and Paz-Chinchón, F and Plazas, A A and Sanchez, E and Scarpine, V and Serrano, S and Sevilla-Noarbe, I and Smith, M and Soares-Santos, M and Sobreira, F and Swanson, M E C and Tarle, G and Vikram, V and (DES Collaboration)},
    title = "{Search for RR Lyrae stars in DES ultrafaint systems: Grus I, Kim 2, Phoenix II, and Grus II}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {490},
    number = {2},
    pages = {2183-2199},
    year = {2019},
    month = {09},
    issn = {0035-8711},
    doi = {10.1093/mnras/stz2609},
    url = {https://doi.org/10.1093/mnras/stz2609},
    eprint = {https://academic.oup.com/mnras/article-pdf/490/2/2183/30257315/stz2609.pdf},
}




@ARTICLE{2017MNRAS.465..472K,
       author = {{Karim}, M.~T. and {Mamajek}, Eric E.},
        title = "{Revised geometric estimates of the North Galactic Pole and the Sun's height above the Galactic mid-plane}",
      journal = {\mnras},
     keywords = {Galaxy: centre, Galaxy: disc- Galaxy: fundamental parameters, Galaxy: general, Galaxy: kinematics and dynamics, Galaxy: structure, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = feb,
       volume = {465},
       number = {1},
        pages = {472-481},
          doi = {10.1093/mnras/stw2772},
archivePrefix = {arXiv},
       eprint = {1610.08125},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.465..472K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019MNRAS.482..921S,
       author = {{Simion}, Iulia T. and {Belokurov}, Vasily and {Koposov}, Sergey E.},
        title = "{Common origin for Hercules-Aquila and Virgo Clouds in Gaia DR2}",
      journal = {\mnras},
     keywords = {Galaxy: formation, Galaxy: structure, galaxies: individual: Milky Way, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jan,
       volume = {482},
       number = {1},
        pages = {921-928},
          doi = {10.1093/mnras/sty2744},
archivePrefix = {arXiv},
       eprint = {1807.01335},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.482..921S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2020MNRAS.494.3880B,
       author = {{Belokurov}, Vasily and {Sanders}, Jason L. and {Fattahi}, Azadeh and {Smith}, Martin C. and {Deason}, Alis J. and {Evans}, N. Wyn and {Grand}, Robert J.~J.},
        title = "{The biggest splash}",
      journal = {\mnras},
     keywords = {Galaxy: formation, Galaxy: halo, galaxies: dwarf, Local Group, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = may,
       volume = {494},
       number = {3},
        pages = {3880-3898},
          doi = {10.1093/mnras/staa876},
archivePrefix = {arXiv},
       eprint = {1909.04679},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.3880B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2018MNRAS.476.3913S,
       author = {{Simion}, Iulia T. and {Belokurov}, Vasily and {Koposov}, Sergey E. and {Sheffield}, Allyson and {Johnston}, Kathryn V.},
        title = "{Spectroscopic follow-up of the Hercules-Aquila Cloud}",
      journal = {\mnras},
     keywords = {Galaxy: formation, Galaxy: halo, Galaxy: structure, galaxies: individual: Milky Way, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = may,
       volume = {476},
       number = {3},
        pages = {3913-3923},
          doi = {10.1093/mnras/sty499},
archivePrefix = {arXiv},
       eprint = {1803.05918},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.3913S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2017ApJ...850...96H,
       author = {{Hernitschek}, Nina and {Sesar}, Branimir and {Rix}, Hans-Walter and {Belokurov}, Vasily and {Martinez-Delgado}, David and {Martin}, Nicolas F. and {Kaiser}, Nick and {Hodapp}, Klaus and {Chambers}, Kenneth C. and {Wainscoat}, Richard and {Magnier}, Eugene and {Kudritzki}, Rolf-Peter and {Metcalfe}, Nigel and {Draper}, Peter W.},
        title = "{The Geometry of the Sagittarius Stream from Pan-STARRS1 3{\ensuremath{\pi}} RR Lyrae}",
      journal = {\apj},
     keywords = {galaxies: dwarf, stars: variables: RR Lyrae, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = nov,
       volume = {850},
       number = {1},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/aa960c},
archivePrefix = {arXiv},
       eprint = {1710.09436},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...850...96H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2018MNRAS.477.1472B,
       author = {{Belokurov}, V. and {Deason}, A.~J. and {Koposov}, S.~E. and {Catelan}, M. and {Erkal}, D. and {Drake}, A.~J. and {Evans}, N.~W.},
        title = "{Unmixing the Galactic halo with RR Lyrae tagging}",
      journal = {\mnras},
     keywords = {stars: variables: RR Lyrae, galaxies: dwarf, Local Group, galaxies: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jun,
       volume = {477},
       number = {2},
        pages = {1472-1483},
          doi = {10.1093/mnras/sty615},
archivePrefix = {arXiv},
       eprint = {1711.07485},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.477.1472B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{Homma_2016,
	doi = {10.3847/0004-637x/832/1/21},
	url = {https://doi.org/10.3847%2F0004-637x%2F832%2F1%2F21},
	year = 2016,
	month = {nov},
	publisher = {American Astronomical Society},
	volume = {832},
	number = {1},
	pages = {21},
	author = {Daisuke Homma and Masashi Chiba and Sakurako Okamoto and Yutaka Komiyama and Masayuki Tanaka and Mikito Tanaka and Miho N. Ishigaki and Masayuki Akiyama and Nobuo Arimoto and Jos{\'{e}} A. Garmilla and Robert H. Lupton and Michael A. Strauss and Hisanori Furusawa and Satoshi Miyazaki and Hitoshi Murayama and Atsushi J. Nishizawa and Masahiro Takada and Tomonori Usuda and Shiang-Yu Wang},
	title = {A {NEW} {MILKY} {WAY} {SATELLITE} {DISCOVERED} {IN} {THE} {SUBARU}/{HYPER} {SUPRIME}-{CAM} {SURVEY}},
	journal = {The Astrophysical Journal}
}



@ARTICLE{2018AA...620A.155M,
       author = {{Massari}, D. and {Helmi}, A.},
        title = "{With and without spectroscopy: Gaia DR2 proper motions of seven ultra-faint dwarf galaxies}",
      journal = {\aap},
     keywords = {Galaxy: kinematics and dynamics, galaxies: dwarf, Local Group, astrometry, proper motions, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = dec,
       volume = {620},
          eid = {A155},
        pages = {A155},
          doi = {10.1051/0004-6361/201833367},
archivePrefix = {arXiv},
       eprint = {1805.01839},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...620A.155M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2012AJ....144....4M,
       author = {{McConnachie}, Alan W.},
        title = "{The Observed Properties of Dwarf Galaxies in and around the Local Group}",
      journal = {\aj},
     keywords = {catalogs, galaxies: dwarf, galaxies: fundamental parameters, galaxies: general, galaxies: structure, Local Group, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = jul,
       volume = {144},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1088/0004-6256/144/1/4},
archivePrefix = {arXiv},
       eprint = {1204.1562},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AJ....144....4M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021arXiv210409794B,
       author = {{Balbinot}, E. and {Helmi}, A.},
        title = "{Linking nearby stellar streams to more distant halo overdensities}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
          eid = {arXiv:2104.09794},
        pages = {arXiv:2104.09794},
archivePrefix = {arXiv},
       eprint = {2104.09794},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210409794B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2016ApJ...817..135L,
       author = {{Li}, T.~S. and {Balbinot}, E. and {Mondrik}, N. and {Marshall}, J.~L. and {Yanny}, B. and {Bechtol}, K. and {Drlica-Wagner}, A. and {Oscar}, D. and {Santiago}, B. and {Simon}, J.~D. and {Vivas}, A.~K. and {Walker}, A.~R. and {Wang}, M.~Y. and {Abbott}, T.~M.~C. and {Abdalla}, F.~B. and {Benoit-L{\'e}vy}, A. and {Bernstein}, G.~M. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {da Costa}, L.~N. and {DePoy}, D.~L. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Estrada}, J. and {Finley}, D.~A. and {Flaugher}, B. and {Frieman}, J. and {Gruen}, D. and {Gruendl}, R.~A. and {Gutierrez}, G. and {Honscheid}, K. and {James}, D.~J. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Maia}, M.~A.~G. and {March}, M. and {Martini}, P. and {Ogando}, R. and {Plazas}, A.~A. and {Reil}, K. and {Romer}, A.~K. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Sevilla-Noarbe}, I. and {Smith}, R.~C. and {Soares-Santos}, M. and {Sobreira}, F. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Tucker}, D. and {Zhang}, Y. and {DES Collaboration}},
        title = "{Discovery of a Stellar Overdensity in Eridanus-Phoenix in the Dark Energy Survey}",
      journal = {\apj},
     keywords = {galaxy: formation, galaxy: halo, galaxy: structure, local group, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = feb,
       volume = {817},
       number = {2},
          eid = {135},
        pages = {135},
          doi = {10.3847/0004-637X/817/2/135},
archivePrefix = {arXiv},
       eprint = {1509.04296},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...817..135L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009ApJ...696..870D,
       author = {{Drake}, A.~J. and {Djorgovski}, S.~G. and {Mahabal}, A. and {Beshore}, E. and {Larson}, S. and {Graham}, M.~J. and {Williams}, R. and {Christensen}, E. and {Catelan}, M. and {Boattini}, A. and {Gibbs}, A. and {Hill}, R. and {Kowalski}, R.},
        title = "{First Results from the Catalina Real-Time Transient Survey}",
      journal = {\apj},
     keywords = {BL Lacertae objects: general, galaxies: general, novae, cataclysmic variables, stars: flare, supernovae: general, Astrophysics},
         year = 2009,
        month = may,
       volume = {696},
       number = {1},
        pages = {870-884},
          doi = {10.1088/0004-637X/696/1/870},
archivePrefix = {arXiv},
       eprint = {0809.1394},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...696..870D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2015AcA....65....1U,
       author = {{Udalski}, A. and {Szyma{\'n}ski}, M.~K. and {Szyma{\'n}ski}, G.},
        title = "{OGLE-IV: Fourth Phase of the Optical Gravitational Lensing Experiment}",
      journal = {\actaa},
     keywords = {Surveys, Techniques: Photometric, Galaxy: bulge, Galaxy: disk, Magellanic Clouds, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2015,
        month = mar,
       volume = {65},
       number = {1},
        pages = {1-38},
archivePrefix = {arXiv},
       eprint = {1504.05966},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015AcA....65....1U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2017PASP..129j4502K,
       author = {{Kochanek}, C.~S. and {Shappee}, B.~J. and {Stanek}, K.~Z. and {Holoien}, T.~W. -S. and {Thompson}, Todd A. and {Prieto}, J.~L. and {Dong}, Subo and {Shields}, J.~V. and {Will}, D. and {Britt}, C. and {Perzanowski}, D. and {Pojma{\'n}ski}, G.},
        title = "{The All-Sky Automated Survey for Supernovae (ASAS-SN) Light Curve Server v1.0}",
      journal = {\pasp},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = oct,
       volume = {129},
       number = {980},
        pages = {104502},
          doi = {10.1088/1538-3873/aa80d9},
archivePrefix = {arXiv},
       eprint = {1706.07060},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017PASP..129j4502K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2006MNRAS.368.1757W,
       author = {{Wils}, Patrick and {Lloyd}, Christopher and {Bernhard}, Klaus},
        title = "{A catalogue of RR Lyrae stars from the Northern Sky Variability Survey}",
      journal = {\mnras},
     keywords = {Astrophysics},
         year = 2006,
        month = jun,
       volume = {368},
       number = {4},
        pages = {1757-1763},
          doi = {10.1111/j.1365-2966.2006.10236.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0601432},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.368.1757W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{2019AcA....69..321S,
       author = {{Soszy{\'n}ski}, I. and {Udalski}, A. and {Wrona}, M. and {Szyma{\'n}ski}, M.~K. and {Pietrukowicz}, P. and {Skowron}, J. and {Skowron}, D. and {Poleski}, R. and {Koz{\l}owski}, S. and {Mr{\'o}z}, P. and {Ulaczyk}, K. and {Rybicki}, K. and {Iwanek}, P. and {Gromadzki}, M.},
        title = "{Over 78 000 RR Lyrae Stars in the Galactic Bulge and Disk from the OGLE Survey}",
      journal = {\actaa},
     keywords = {Stars: variables: RR Lyrae, Stars: oscillations, Galaxy: bulge, Galaxy: disk, Catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = dec,
       volume = {69},
       number = {4},
        pages = {321-337},
          doi = {10.32023/0001-5237/69.4.2},
archivePrefix = {arXiv},
       eprint = {2001.00025},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AcA....69..321S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{2018ApJ...859...31H,
       author = {{Hernitschek}, Nina and {Cohen}, Judith G. and {Rix}, Hans-Walter and {Sesar}, Branimir and {Martin}, Nicolas F. and {Magnier}, Eugene and {Wainscoat}, Richard and {Kaiser}, Nick and {Tonry}, John L. and {Kudritzki}, Rolf-Peter and {Hodapp}, Klaus and {Chambers}, Ken and {Flewelling}, Heather and {Burgett}, William},
        title = "{The Profile of the Galactic Halo from Pan-STARRS1 3{\ensuremath{\pi}} RR Lyrae}",
      journal = {\apj},
     keywords = {Galaxy: halo, stars: variables: RR Lyrae, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = may,
       volume = {859},
       number = {1},
          eid = {31},
        pages = {31},
          doi = {10.3847/1538-4357/aabfbb},
archivePrefix = {arXiv},
       eprint = {1801.10260},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...859...31H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2018A&A...618A..30H,
       author = {{Holl}, B. and {Audard}, M. and {Nienartowicz}, K. and {Jevardat de Fombelle}, G. and {Marchal}, O. and {Mowlavi}, N. and {Clementini}, G. and {De Ridder}, J. and {Evans}, D.~W. and {Guy}, L.~P. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {Rimoldini}, L. and {Roelens}, M. and {Zucker}, S. and {Distefano}, E. and {Garofalo}, A. and {Lecoeur-Ta{\"\i}bi}, I. and {Lopez}, M. and {Molinaro}, R. and {Muraveva}, T. and {Panahi}, A. and {Regibo}, S. and {Ripepi}, V. and {Sarro}, L.~M. and {Aerts}, C. and {Anderson}, R.~I. and {Charnas}, J. and {Barblan}, F. and {Blanco-Cuaresma}, S. and {Busso}, G. and {Cuypers}, J. and {De Angeli}, F. and {Glass}, F. and {Grenon}, M. and {Juh{\'a}sz}, {\'A}. L. and {Kochoska}, A. and {Koubsky}, P. and {Lanza}, A.~F. and {Leccia}, S. and {Lorenz}, D. and {Marconi}, M. and {Marschalk{\'o}}, G. and {Mazeh}, T. and {Messina}, S. and {Mignard}, F. and {Moitinho}, A. and {Moln{\'a}r}, L. and {Morgenthaler}, S. and {Musella}, I. and {Ordenovic}, C. and {Ord{\'o}{\~n}ez}, D. and {Pagano}, I. and {Palaversa}, L. and {Pawlak}, M. and {Plachy}, E. and {Pr{\v{s}}a}, A. and {Riello}, M. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Votruba}, V. and {Eyer}, L.},
        title = "{Gaia Data Release 2. Summary of the variability processing and analysis results}",
      journal = {\aap},
     keywords = {stars: general, stars: oscillations, stars: solar-type, stars: variables: general, Galaxy: stellar content, catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A30},
        pages = {A30},
          doi = {10.1051/0004-6361/201832892},
archivePrefix = {arXiv},
       eprint = {1804.09373},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A..30H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018AA...618A..30H,
       author = {{Holl}, B. and {Audard}, M. and {Nienartowicz}, K. and {Jevardat de Fombelle}, G. and {Marchal}, O. and {Mowlavi}, N. and {Clementini}, G. and {De Ridder}, J. and {Evans}, D.~W. and {Guy}, L.~P. and {Lanzafame}, A.~C. and {Lebzelter}, T. and {Rimoldini}, L. and {Roelens}, M. and {Zucker}, S. and {Distefano}, E. and {Garofalo}, A. and {Lecoeur-Ta{\"\i}bi}, I. and {Lopez}, M. and {Molinaro}, R. and {Muraveva}, T. and {Panahi}, A. and {Regibo}, S. and {Ripepi}, V. and {Sarro}, L.~M. and {Aerts}, C. and {Anderson}, R.~I. and {Charnas}, J. and {Barblan}, F. and {Blanco-Cuaresma}, S. and {Busso}, G. and {Cuypers}, J. and {De Angeli}, F. and {Glass}, F. and {Grenon}, M. and {Juh{\'a}sz}, {\'A}. L. and {Kochoska}, A. and {Koubsky}, P. and {Lanza}, A.~F. and {Leccia}, S. and {Lorenz}, D. and {Marconi}, M. and {Marschalk{\'o}}, G. and {Mazeh}, T. and {Messina}, S. and {Mignard}, F. and {Moitinho}, A. and {Moln{\'a}r}, L. and {Morgenthaler}, S. and {Musella}, I. and {Ordenovic}, C. and {Ord{\'o}{\~n}ez}, D. and {Pagano}, I. and {Palaversa}, L. and {Pawlak}, M. and {Plachy}, E. and {Pr{\v{s}}a}, A. and {Riello}, M. and {S{\"u}veges}, M. and {Szabados}, L. and {Szegedi-Elek}, E. and {Votruba}, V. and {Eyer}, L.},
        title = "{Gaia Data Release 2. Summary of the variability processing and analysis results}",
      journal = {\aap},
     keywords = {stars: general, stars: oscillations, stars: solar-type, stars: variables: general, Galaxy: stellar content, catalogs, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = oct,
       volume = {618},
          eid = {A30},
        pages = {A30},
          doi = {10.1051/0004-6361/201832892},
archivePrefix = {arXiv},
       eprint = {1804.09373},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...618A..30H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2014MNRAS.440..161S,
       author = {{Simion}, Iulia T. and {Belokurov}, Vasily and {Irwin}, Mike and {Koposov}, Sergey E.},
        title = "{Strong RR Lyrae excess in the Hercules-Aquila Cloud}",
      journal = {\mnras},
     keywords = {stars: variables: RR Lyrae, Galaxy: halo, Galaxy: stellar content, Galaxy: structure, galaxies: individual: Milky Way, galaxies: photometry, Astrophysics - Galaxy Astrophysics},
         year = 2014,
        month = may,
       volume = {440},
       number = {1},
        pages = {161-171},
          doi = {10.1093/mnras/stu133},
archivePrefix = {arXiv},
       eprint = {1401.4354},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.440..161S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2007ApJ...657L..89B,
       author = {{Belokurov}, V. and {Evans}, N.~W. and {Bell}, E.~F. and {Irwin}, M.~J. and {Hewett}, P.~C. and {Koposov}, S. and {Rockosi}, C.~M. and {Gilmore}, G. and {Zucker}, D.~B. and {Fellhauer}, M. and {Wilkinson}, M.~I. and {Bramich}, D.~M. and {Vidrih}, S. and {Rix}, H. -W. and {Beers}, T.~C. and {Schneider}, D.~P. and {Barentine}, J.~C. and {Brewington}, H. and {Brinkmann}, J. and {Harvanek}, M. and {Krzesinski}, J. and {Long}, D. and {Pan}, K. and {Snedden}, S.~A. and {Malanushenko}, O. and {Malanushenko}, V.},
        title = "{The Hercules-Aquila Cloud}",
      journal = {\apjl},
     keywords = {Galaxies: Kinematics and Dynamics, Galaxies: Structure, Galaxy: Halo, Galaxies: Local Group, Astrophysics},
         year = 2007,
        month = mar,
       volume = {657},
       number = {2},
        pages = {L89-L92},
          doi = {10.1086/513144},
archivePrefix = {arXiv},
       eprint = {astro-ph/0701790},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...657L..89B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2012AJ....143..105B,
       author = {{Bonaca}, Ana and {Juri{\'c}}, Mario and {Ivezi{\'c}}, {\v{Z}}eljko and {Bizyaev}, Dmitry and {Brewington}, Howard and {Malanushenko}, Elena and {Malanushenko}, Viktor and {Oravetz}, Daniel and {Pan}, Kaike and {Shelden}, Alaina and {Simmons}, Audrey and {Snedden}, Stephanie},
        title = "{Update on the Nature of Virgo Overdensity}",
      journal = {\aj},
     keywords = {Galaxy: formation, Galaxy: halo, Galaxy: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = may,
       volume = {143},
       number = {5},
          eid = {105},
        pages = {105},
          doi = {10.1088/0004-6256/143/5/105},
archivePrefix = {arXiv},
       eprint = {1202.6367},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012AJ....143..105B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2008ApJ...673..864J,
       author = {{Juri{\'c}}, Mario and {Ivezi{\'c}}, {\v{Z}}eljko and {Brooks}, Alyson and {Lupton}, Robert H. and {Schlegel}, David and {Finkbeiner}, Douglas and {Padmanabhan}, Nikhil and {Bond}, Nicholas and {Sesar}, Branimir and {Rockosi}, Constance M. and {Knapp}, Gillian R. and {Gunn}, James E. and {Sumi}, Takahiro and {Schneider}, Donald P. and {Barentine}, J.~C. and {Brewington}, Howard J. and {Brinkmann}, J. and {Fukugita}, Masataka and {Harvanek}, Michael and {Kleinman}, S.~J. and {Krzesinski}, Jurek and {Long}, Dan and {Neilsen}, Eric H., Jr. and {Nitta}, Atsuko and {Snedden}, Stephanie A. and {York}, Donald G.},
        title = "{The Milky Way Tomography with SDSS. I. Stellar Number Density Distribution}",
      journal = {\apj},
     keywords = {Galaxy: disk, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: structure, Astrophysics},
         year = 2008,
        month = feb,
       volume = {673},
       number = {2},
        pages = {864-914},
          doi = {10.1086/523619},
archivePrefix = {arXiv},
       eprint = {astro-ph/0510520},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...673..864J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2006ApJ...636L..97D,
       author = {{Duffau}, Sonia and {Zinn}, Robert and {Vivas}, A. Katherina and {Carraro}, Giovanni and {M{\'e}ndez}, Ren{\'e} A. and {Winnick}, Rebeccah and {Gallart}, Carme},
        title = "{Spectroscopy of QUEST RR Lyrae Variables: The New Virgo Stellar Stream}",
      journal = {\apjl},
     keywords = {Galaxy: Halo, Galaxy: Kinematics and Dynamics, Galaxy: Structure, Stars: Variables: Other, Astrophysics},
         year = 2006,
        month = jan,
       volume = {636},
       number = {2},
        pages = {L97-L100},
          doi = {10.1086/500130},
archivePrefix = {arXiv},
       eprint = {astro-ph/0510589},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...636L..97D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018ApJ...855...43M,
       author = {{Medina}, Gustavo E. and {Mu{\~n}oz}, Ricardo R. and {Vivas}, A. Katherina and {Carlin}, Jeffrey L. and {F{\"o}rster}, Francisco and {Mart{\'\i}nez}, Jorge and {Galbany}, Llu{\'\i}s and {Gonz{\'a}lez-Gait{\'a}n}, Santiago and {Hamuy}, Mario and {de Jaeger}, Thomas and {Maureira}, Juan Carlos and {San Mart{\'\i}n}, Jaime},
        title = "{Discovery of Distant RR Lyrae Stars in the Milky Way Using DECam}",
      journal = {\apj},
     keywords = {Galaxy: halo, Galaxy: stellar content, Galaxy: structure, stars: variables: RR Lyrae, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = mar,
       volume = {855},
       number = {1},
          eid = {43},
        pages = {43},
          doi = {10.3847/1538-4357/aaad02},
archivePrefix = {arXiv},
       eprint = {1802.01581},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...855...43M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2021ApJ...911..109S,
       author = {{Stringer}, K.~M. and {Drlica-Wagner}, A. and {Macri}, L. and {Mart{\'\i}nez-V{\'a}zquez}, C.~E. and {Vivas}, A.~K. and {Ferguson}, P. and {Pace}, A.~B. and {Walker}, A.~R. and {Neilsen}, E. and {Tavangar}, K. and {Wester}, W. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Bacon}, D. and {Bechtol}, K. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Ferrero}, I. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Kuehn}, K. and {Kuropatkin}, N. and {Li}, T.~S. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Roodman}, A. and {Sanchez}, E. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Wilkinson}, R.~D. and {Zhang}, Y. and {DES Collaboration}},
        title = "{Identifying RR Lyrae Variable Stars in Six Years of the Dark Energy Survey}",
      journal = {\apj},
     keywords = {RR Lyrae variable stars, RRab variable stars, Milky Way stellar halo, the Milky Way, 1410, 1413, 1060, 1054, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = apr,
       volume = {911},
       number = {2},
          eid = {109},
        pages = {109},
          doi = {10.3847/1538-4357/abe873},
archivePrefix = {arXiv},
       eprint = {2011.13930},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911..109S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2002ApJ...569..245N,
       author = {{Newberg}, Heidi Jo and {Yanny}, Brian and {Rockosi}, Connie and {Grebel}, Eva K. and {Rix}, Hans-Walter and {Brinkmann}, Jon and {Csabai}, Istvan and {Hennessy}, Greg and {Hindsley}, Robert B. and {Ibata}, Rodrigo and {Ivezi{\'c}}, Zeljko and {Lamb}, Don and {Nash}, E. Thomas and {Odenkirchen}, Michael and {Rave}, Heather A. and {Schneider}, D.~P. and {Smith}, J. Allyn and {Stolte}, Andrea and {York}, Donald G.},
        title = "{The Ghost of Sagittarius and Lumps in the Halo of the Milky Way}",
      journal = {\apj},
     keywords = {Galaxy: Halo, Galaxy: Structure, Astrophysics},
         year = 2002,
        month = apr,
       volume = {569},
       number = {1},
        pages = {245-274},
          doi = {10.1086/338983},
archivePrefix = {arXiv},
       eprint = {astro-ph/0111095},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...569..245N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2001ApJ...554L..33V,
       author = {{Vivas}, A.~K. and {Zinn}, R. and {Andrews}, P. and {Bailyn}, C. and {Baltay}, C. and {Coppi}, P. and {Ellman}, N. and {Girard}, T. and {Rabinowitz}, D. and {Schaefer}, B. and {Shin}, J. and {Snyder}, J. and {Sofia}, S. and {van Altena}, W. and {Abad}, C. and {Bongiovanni}, A. and {Brice{\~n}o}, C. and {Bruzual}, G. and {Della Prugna}, F. and {Herrera}, D. and {Magris}, G. and {Mateu}, J. and {Pacheco}, R. and {S{\'a}nchez}, Ge. and {S{\'a}nchez}, Gu. and {Schenner}, H. and {Stock}, J. and {Vicente}, B. and {Vieira}, K. and {Ferr{\'\i}n}, I. and {Hernandez}, J. and {Gebhard}, M. and {Honeycutt}, R. and {Mufson}, S. and {Musser}, J. and {Rengstorf}, A.},
        title = "{The QUEST RR Lyrae Survey: Confirmation of the Clump at 50 Kiloparsecs and Other Overdensities in the Outer Halo}",
      journal = {\apjl},
     keywords = {Galaxies: Individual: Name: Sagittarius, Galaxy: Halo, Galaxy: Structure, Stars: Variables: Other, Astrophysics},
         year = 2001,
        month = jun,
       volume = {554},
       number = {1},
        pages = {L33-L36},
          doi = {10.1086/320915},
archivePrefix = {arXiv},
       eprint = {astro-ph/0105135},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...554L..33V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2019MNRAS.482.3868I,
       author = {{Iorio}, Giuliano and {Belokurov}, Vasily},
        title = "{The shape of the Galactic halo with Gaia DR2 RR Lyrae. Anatomy of an ancient major merger}",
      journal = {\mnras},
     keywords = {stars: variables: RR Lyrae, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure, galaxies: individual (Milky Way), Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = jan,
       volume = {482},
       number = {3},
        pages = {3868-3879},
          doi = {10.1093/mnras/sty2806},
archivePrefix = {arXiv},
       eprint = {1808.04370},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.482.3868I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1999AJ....118.1373L,
       author = {{Lee}, Jae-Woo and {Carney}, Bruce W.},
        title = "{RR Lyrae Luminosity Differences between Oosterhoff Group I and II Cluster Systems and the Origin of the Oosterhoff Dichotomy}",
      journal = {\aj},
     keywords = {GALAXY: FORMATION-GLOBULAR CLUSTERS: INDIVIDUAL (NGC 5272, NGC 7089), STARS: VARIABLES: RR LYRAE VARIABLE, STARS: HORIZONTAL-BRANCH, STARS: LUMINOSITY FUNCTION, MASS FUNCTION},
         year = 1999,
        month = sep,
       volume = {118},
       number = {3},
        pages = {1373-1389},
          doi = {10.1086/301008},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999AJ....118.1373L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1973ApJ...185..477V,
       author = {{van Albada}, T.~S. and {Baker}, Norman},
        title = "{On the Two Oosterhoff Groups of Globular Clusters}",
      journal = {\apj},
         year = 1973,
        month = oct,
       volume = {185},
        pages = {477-498},
          doi = {10.1086/152434},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973ApJ...185..477V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2018MNRAS.474.2142I,
       author = {{Iorio}, G. and {Belokurov}, V. and {Erkal}, D. and {Koposov}, S.~E. and {Nipoti}, C. and {Fraternali}, F.},
        title = "{The first all-sky view of the Milky Way stellar halo with Gaia+2MASS RR Lyrae}",
      journal = {\mnras},
     keywords = {stars: variables: RR Lyrae, Galaxy: halo, Galaxy: stellar content, Galaxy: structure, galaxies: individual: Milky Way, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = feb,
       volume = {474},
       number = {2},
        pages = {2142-2166},
          doi = {10.1093/mnras/stx2819},
archivePrefix = {arXiv},
       eprint = {1707.03833},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.474.2142I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{1907AN....175..325B,
       author = {{Bla{\v{z}}ko}, S.},
        title = "{Mitteilung {\"u}ber ver{\"a}nderliche Sterne}",
      journal = {Astronomische Nachrichten},
         year = 1907,
        month = aug,
       volume = {175},
        pages = {325},
          doi = {10.1002/asna.19071752002},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1907AN....175..325B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{Sesar_2014,
	doi = {10.1088/0004-637x/793/2/135},
	url = {https://doi.org/10.1088/0004-637x/793/2/135},
	year = 2014,
	month = {sep},
	publisher = {American Astronomical Society},
	volume = {793},
	number = {2},
	pages = {135},
	author = {Branimir Sesar and Sophianna R. Banholzer and Judith G. Cohen and Nicolas F. Martin and Carl J. Grillmair and David Levitan and Russ R. Laher and Eran O. Ofek and Jason A. Surace and Shrinivas R. Kulkarni and Thomas A. Prince and Hans-Walter Rix},
	title = {{STACKING} {THE} {INVISIBLES}: A {GUIDED} {SEARCH} {FOR} {LOW}-{LUMINOSITY} {MILKY} {WAY} {SATELLITES}},
	journal = {The Astrophysical Journal}
}


@article{C_ceres_2008,
	doi = {10.1086/591231},
	url = {https://doi.org/10.1086/591231},
	year = 2008,
	month = {nov},
	publisher = {American Astronomical Society},
	volume = {179},
	number = {1},
	pages = {242--248},
	author = {C. C{\'{a}}ceres and M. Catelan},
	title = {The Period-Luminosity Relation of {RR} Lyrae Stars in the {SDSS} Photometric System},
	journal = {The Astrophysical Journal Supplement Series},
	abstract = {We provide the first detailed study of the RR Lyrae period-luminosity (PL) relation in the ugriz bandpasses of the Sloan Digital Sky Survey (SDSS) filter system. We argue that tight, simple PL relations are not present in the SDSS filters, except for the redder bandpasses i  and (especially) z. However, for all bandpasses, we show that by incorporating terms involving a (fairly reddening-independent) “pseudocolor” C0 ≡ (u − g)0 − (g − r)0, we can obtain tight (nonlinear) relations. We provide such theoretically calibrated relations in the present paper, which should be useful in deriving precise absolute magnitudes (hence distances) and intrinsic colors (hence reddening values) even to individual field RR Lyrae stars. For applications to cases in which photometry in all five passbands may not be available, we also provide simple (although less precise) average PL relations for the i and z bandpasses, which read as


 and


 Similarly, simple period-color relations for (r − i)0, (g − r)0, and (u − z)0 are also provided.}
}


@article{Baker_2015,
	doi = {10.1088/0004-6256/150/5/160},
	url = {https://doi.org/10.1088/0004-6256/150/5/160},
	year = 2015,
	month = {oct},
	publisher = {American Astronomical Society},
	volume = {150},
	number = {5},
	pages = {160},
	author = {Mariah Baker and Beth Willman},
	title = {{CHARTING} {UNEXPLORED} {DWARF} {GALAXY} {TERRITORY} {WITH} {RR} {LYRAE}},
	journal = {The Astronomical Journal}
}



@ARTICLE{2012MSAIS..19..138M,
       author = {{Marconi}, M.},
        title = "{RR Lyrae pulsating stars as stellar population tracers and distance indicators .}",
      journal = {Memorie della Societa Astronomica Italiana Supplementi},
     keywords = {Stars: RR Lyrae, Stars: distances, Stars: Population II},
         year = 2012,
        month = jan,
       volume = {19},
        pages = {138},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MSAIS..19..138M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@Inbook{Cacciari2003,
author="Cacciari, Carla and Clementini, Gisella",
editor="Alloin, Danielle and Gieren, Wolfgang",
title="Globular Cluster Distances from RR Lyrae Stars",
bookTitle="Stellar Candles for the Extragalactic Distance Scale",
year="2003",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="105--122",
abstract="The most common methods to derive the distance to globular clusters using RR Lyrae variables are reviewed, with a special attention to those that have experienced significant improvement in the past few years. From the weighted average of these most recent determinations the absolute magnitude of the RR Lyrae stars at [Fe/H] = −1.5 is MV= 0.59 {\textpm} 0.03, corresponding to a distance modulus for the LMC (m − M)0 = 18.48 {\textpm} 0.05.",
isbn="978-3-540-39882-0",
doi="10.1007/978-3-540-39882-0_6",
url="https://doi.org/10.1007/978-3-540-39882-0_6"
}




@ARTICLE{1995CAS....27.....S,
       author = {{Smith}, H.~A.},
        title = "{RR Lyrae stars.}",
      journal = {Cambridge Astrophysics Series},
     keywords = {RR Lyrae Stars, RR Lyrae Stars: Globular Clusters, RR Lyrae Stars: Galaxies},
         year = 1995,
        month = jan,
       volume = {27},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995CAS....27.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018RNAAS...2...18J,
       author = {{Jayasinghe}, T. and {Kochanek}, C.~S. and {Stanek}, K.~Z. and {Shappee}, B.~J. and {Holoien}, T.~W. -S. and {Thompson}, T.~A. and {Prieto}, J.~L. and {Dong}, Subo and {Britt}, C.~A. and {Will}, D.},
        title = "{ASAS-SN Discovery of 4880 Bright RR Lyrae Variable Stars}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = jan,
       volume = {2},
       number = {1},
          eid = {18},
        pages = {18},
          doi = {10.3847/2515-5172/aaaa20},
archivePrefix = {arXiv},
       eprint = {1801.07716},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018RNAAS...2...18J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2020yCat.2366....0J,
       author = {{Jayasinghe}, T. and {Kochanek}, C.~S. and {Stanek}, K.~Z. and {Shappee}, B.~J. and {Holoien}, T.~W. -S. and {Thompson}, T.~A. and {Prieto}, J.~L. and {Dong}, S. and {Pawlak}, M. and {Shields}, J.~V. and {Pojmanski}, G. and {Otero}, S. and {Britt}, C.~A. and {Will}, D.},
        title = "{VizieR Online Data Catalog: ASAS-SN catalog of variable stars (Jayasinghe+, 2018-2020)}",
      journal = {VizieR Online Data Catalog},
     keywords = {Stars: variable, Photometry: UBVRI, Cross identifications, Proper motions, Surveys},
         year = 2020,
        month = oct,
          eid = {II/366},
        pages = {II/366},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020yCat.2366....0J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019MNRAS.488.2743T,
       author = {{Torrealba}, G. and {Belokurov}, V. and {Koposov}, S.~E. and {Li}, T.~S. and {Walker}, M.~G. and {Sanders}, J.~L. and {Geringer-Sameth}, A. and {Zucker}, D.~B. and {Kuehn}, K. and {Evans}, N.~W. and {Dehnen}, W.},
        title = "{The hidden giant: discovery of an enormous Galactic dwarf satellite in Gaia DR2}",
      journal = {\mnras},
     keywords = {Galaxy: halo, galaxies: dwarf, galaxies: individual: Antlia 2 Dwarf, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = sep,
       volume = {488},
       number = {2},
        pages = {2743-2766},
          doi = {10.1093/mnras/stz1624},
archivePrefix = {arXiv},
       eprint = {1811.04082},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.488.2743T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1998AJ....115.1135R,
       author = {{Rucinski}, Slavek M.},
        title = "{Eclipsing Binaries in the OGLE Variable Star Catalog. III. Long-Period Contact Systems}",
      journal = {\aj},
     keywords = {BINARIES: ECLIPSING, Astrophysics},
         year = 1998,
        month = mar,
       volume = {115},
       number = {3},
        pages = {1135-1144},
          doi = {10.1086/300266},
archivePrefix = {arXiv},
       eprint = {astro-ph/9711317},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998AJ....115.1135R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2008ApJ...684..287I,
       author = {{Ivezi{\'c}}, {\v{Z}}eljko and {Sesar}, Branimir and {Juri{\'c}}, Mario and {Bond}, Nicholas and {Dalcanton}, Julianne and {Rockosi}, Constance M. and {Yanny}, Brian and {Newberg}, Heidi J. and {Beers}, Timothy C. and {Allende Prieto}, Carlos and {Wilhelm}, Ron and {Lee}, Young Sun and {Sivarani}, Thirupathi and {Norris}, John E. and {Bailer-Jones}, Coryn A.~L. and {Re Fiorentin}, Paola and {Schlegel}, David and {Uomoto}, Alan and {Lupton}, Robert H. and {Knapp}, Gillian R. and {Gunn}, James E. and {Covey}, Kevin R. and {Allyn Smith}, J. and {Miknaitis}, Gajus and {Doi}, Mamoru and {Tanaka}, Masayuki and {Fukugita}, Masataka and {Kent}, Steve and {Finkbeiner}, Douglas and {Munn}, Jeffrey A. and {Pier}, Jeffrey R. and {Quinn}, Tom and {Hawley}, Suzanne and {Anderson}, Scott and {Kiuchi}, Furea and {Chen}, Alex and {Bushong}, James and {Sohi}, Harkirat and {Haggard}, Daryl and {Kimball}, Amy and {Barentine}, John and {Brewington}, Howard and {Harvanek}, Mike and {Kleinman}, Scott and {Krzesinski}, Jurek and {Long}, Dan and {Nitta}, Atsuko and {Snedden}, Stephanie and {Lee}, Brian and {Harris}, Hugh and {Brinkmann}, Jonathan and {Schneider}, Donald P. and {York}, Donald G.},
        title = "{The Milky Way Tomography with SDSS. II. Stellar Metallicity}",
      journal = {\apj},
     keywords = {Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: stellar content, Galaxy: structure, methods: data analysis, stars: statistics, Astrophysics},
         year = 2008,
        month = sep,
       volume = {684},
       number = {1},
        pages = {287-325},
          doi = {10.1086/589678},
archivePrefix = {arXiv},
       eprint = {0804.3850},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ApJ...684..287I},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2010ApJ...708..717S,
       author = {{Sesar}, Branimir and {Ivezi{\'c}}, {\v{Z}}eljko and {Grammer}, Skyler H. and {Morgan}, Dylan P. and {Becker}, Andrew C. and {Juri{\'c}}, Mario and {De Lee}, Nathan and {Annis}, James and {Beers}, Timothy C. and {Fan}, Xiaohui and {Lupton}, Robert H. and {Gunn}, James E. and {Knapp}, Gillian R. and {Jiang}, Linhua and {Jester}, Sebastian and {Johnston}, David E. and {Lampeitl}, Hubert},
        title = "{Light Curve Templates and Galactic Distribution of RR Lyrae Stars from Sloan Digital Sky Survey Stripe 82}",
      journal = {\apj},
     keywords = {Galaxy: halo, Galaxy: stellar content, Galaxy: structure, methods: data analysis, stars: horizontal-branch, stars: statistics, stars: variables: other, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = jan,
       volume = {708},
       number = {1},
        pages = {717-741},
          doi = {10.1088/0004-637X/708/1/717},
archivePrefix = {arXiv},
       eprint = {0910.4611},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...708..717S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}






@ARTICLE{2004AJ....128..858S,
       author = {{Sandage}, Allan},
        title = "{The Metallicity Dependence of the Fourier Components of RR Lyrae Light Curves Is the Oosterhoff-Arp-Preston Period Ratio Effect in Disguise}",
      journal = {\aj},
     keywords = {Galaxy: Globular Clusters: General, Stars: Evolution, Stars: Horizontal-Branch, Stars: Variables: Other, Astrophysics},
         year = 2004,
        month = aug,
       volume = {128},
       number = {2},
        pages = {858-868},
          doi = {10.1086/422509},
archivePrefix = {arXiv},
       eprint = {astro-ph/0405480},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004AJ....128..858S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2019PASP..131a8003M,
       author = {{Masci}, Frank J. and {Laher}, Russ R. and {Rusholme}, Ben and {Shupe}, David L. and {Groom}, Steven and {Surace}, Jason and {Jackson}, Edward and {Monkewitz}, Serge and {Beck}, Ron and {Flynn}, David and {Terek}, Scott and {Landry}, Walter and {Hacopians}, Eugean and {Desai}, Vandana and {Howell}, Justin and {Brooke}, Tim and {Imel}, David and {Wachter}, Stefanie and {Ye}, Quan-Zhi and {Lin}, Hsing-Wen and {Cenko}, S. Bradley and {Cunningham}, Virginia and {Rebbapragada}, Umaa and {Bue}, Brian and {Miller}, Adam A. and {Mahabal}, Ashish and {Bellm}, Eric C. and {Patterson}, Maria T. and {Juri{\'c}}, Mario and {Golkhou}, V. Zach and {Ofek}, Eran O. and {Walters}, Richard and {Graham}, Matthew and {Kasliwal}, Mansi M. and {Dekany}, Richard G. and {Kupfer}, Thomas and {Burdge}, Kevin and {Cannella}, Christopher B. and {Barlow}, Tom and {Van Sistine}, Angela and {Giomi}, Matteo and {Fremling}, Christoffer and {Blagorodnova}, Nadejda and {Levitan}, David and {Riddle}, Reed and {Smith}, Roger M. and {Helou}, George and {Prince}, Thomas A. and {Kulkarni}, Shrinivas R.},
        title = "{The Zwicky Transient Facility: Data Processing, Products, and Archive}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018003},
          doi = {10.1088/1538-3873/aae8ac},
archivePrefix = {arXiv},
       eprint = {1902.01872},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8003M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1993ApJ...410..526S,
       author = {{Simon}, Norman R. and {Clement}, Christine M.},
        title = "{A Provisional RR Lyrae Distance Scale}",
      journal = {\apj},
     keywords = {Distance, Globular Clusters, Variable Stars, Astronomical Models, Hydrodynamic Equations, Magellanic Clouds, Stellar Luminosity, Stellar Mass, Stellar Oscillations, Stellar Temperature, Astrophysics, GALAXIES: DISTANCES AND REDSHIFTS, GALAXY: GLOBULAR CLUSTERS: GENERAL, GALAXIES: MAGELLANIC CLOUDS, STARS: DISTANCES, STARS: OSCILLATIONS, STARS: VARIABLES: OTHER RR LYRAE},
         year = 1993,
        month = jun,
       volume = {410},
        pages = {526},
          doi = {10.1086/172771},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...410..526S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1996A&A...312..111J,
       author = {{Jurcsik}, J. and {Kovacs}, G.},
        title = "{Determination of [Fe/H] from the light curves of RR Lyrae stars.}",
      journal = {\aap},
     keywords = {STARS: VARIABLES, STARS: OSCILLATIONS, STARS: HORIZONTAL-BRANCH, STARS: ABUNDANCES, GLOBULAR CLUSTERS: GENERAL},
         year = 1996,
        month = aug,
       volume = {312},
        pages = {111-120},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&A...312..111J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2021MNRAS.500.5009M,
       author = {{Marconi}, M. and {Molinaro}, R. and {Ripepi}, V. and {Leccia}, S. and {Musella}, I. and {De Somma}, G. and {Gatto}, M. and {Moretti}, M.~I.},
        title = "{A theoretical scenario for Galactic RR Lyrae in the Gaia data base: constraints on the parallax offset}",
      journal = {\mnras},
     keywords = {stars: abundances, stars: distances, stars: variables: RR Lyrae, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jan,
       volume = {500},
       number = {4},
        pages = {5009-5023},
          doi = {10.1093/mnras/staa3558},
archivePrefix = {arXiv},
       eprint = {2011.06675},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500.5009M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@article{Zonca2019,
  doi = {10.21105/joss.01298},
  url = {https://doi.org/10.21105/joss.01298},
  year = {2019},
  month = mar,
  publisher = {The Open Journal},
  volume = {4},
  number = {35},
  pages = {1298},
  author = {Andrea Zonca and Leo Singer and Daniel Lenz and Martin Reinecke and Cyrille Rosset and Eric Hivon and Krzysztof Gorski},
  title = {healpy: equal area pixelization and spherical harmonics transforms for data on the sphere in Python},
  journal = {Journal of Open Source Software}
}

@ARTICLE{2005ApJ...622..759G,
   author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and 
	{Wandelt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and 
	{Bartelmann}, M.},
    title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0409513},
 keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical},
     year = 2005,
    month = apr,
   volume = 622,
    pages = {759-771},
      doi = {10.1086/427976},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...622..759G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019A&A...622A..60C,
       author = {{Clementini}, G. and {Ripepi}, V. and {Molinaro}, R. and {Garofalo}, A. and {Muraveva}, T. and {Rimoldini}, L. and {Guy}, L.~P. and {Jevardat de Fombelle}, G. and {Nienartowicz}, K. and {Marchal}, O. and {Audard}, M. and {Holl}, B. and {Leccia}, S. and {Marconi}, M. and {Musella}, I. and {Mowlavi}, N. and {Lecoeur-Taibi}, I. and {Eyer}, L. and {De Ridder}, J. and {Regibo}, S. and {Sarro}, L.~M. and {Szabados}, L. and {Evans}, D.~W. and {Riello}, M.},
        title = "{Gaia Data Release 2. Specific characterisation and validation of all-sky Cepheids and RR Lyrae stars}",
      journal = {\aap},
     keywords = {stars: general, stars: oscillations, stars: variables: Cepheids, stars: variables: RR Lyrae, methods: data analysis, Galaxy: structure, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A60},
        pages = {A60},
          doi = {10.1051/0004-6361/201833374},
archivePrefix = {arXiv},
       eprint = {1805.02079},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A..60C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019AA...622A..60C,
       author = {{Clementini}, G. and {Ripepi}, V. and {Molinaro}, R. and {Garofalo}, A. and {Muraveva}, T. and {Rimoldini}, L. and {Guy}, L.~P. and {Jevardat de Fombelle}, G. and {Nienartowicz}, K. and {Marchal}, O. and {Audard}, M. and {Holl}, B. and {Leccia}, S. and {Marconi}, M. and {Musella}, I. and {Mowlavi}, N. and {Lecoeur-Taibi}, I. and {Eyer}, L. and {De Ridder}, J. and {Regibo}, S. and {Sarro}, L.~M. and {Szabados}, L. and {Evans}, D.~W. and {Riello}, M.},
        title = "{Gaia Data Release 2. Specific characterisation and validation of all-sky Cepheids and RR Lyrae stars}",
      journal = {\aap},
     keywords = {stars: general, stars: oscillations, stars: variables: Cepheids, stars: variables: RR Lyrae, methods: data analysis, Galaxy: structure, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = feb,
       volume = {622},
          eid = {A60},
        pages = {A60},
          doi = {10.1051/0004-6361/201833374},
archivePrefix = {arXiv},
       eprint = {1805.02079},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A..60C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019PASP..131a8002B,
       author = {{Bellm}, Eric C. and {Kulkarni}, Shrinivas R. and {Graham}, Matthew J. and {Dekany}, Richard and {Smith}, Roger M. and {Riddle}, Reed and {Masci}, Frank J. and {Helou}, George and {Prince}, Thomas A. and {Adams}, Scott M. and {Barbarino}, C. and {Barlow}, Tom and {Bauer}, James and {Beck}, Ron and {Belicki}, Justin and {Biswas}, Rahul and {Blagorodnova}, Nadejda and {Bodewits}, Dennis and {Bolin}, Bryce and {Brinnel}, Valery and {Brooke}, Tim and {Bue}, Brian and {Bulla}, Mattia and {Burruss}, Rick and {Cenko}, S. Bradley and {Chang}, Chan-Kao and {Connolly}, Andrew and {Coughlin}, Michael and {Cromer}, John and {Cunningham}, Virginia and {De}, Kishalay and {Delacroix}, Alex and {Desai}, Vandana and {Duev}, Dmitry A. and {Eadie}, Gwendolyn and {Farnham}, Tony L. and {Feeney}, Michael and {Feindt}, Ulrich and {Flynn}, David and {Franckowiak}, Anna and {Frederick}, S. and {Fremling}, C. and {Gal-Yam}, Avishay and {Gezari}, Suvi and {Giomi}, Matteo and {Goldstein}, Daniel A. and {Golkhou}, V. Zach and {Goobar}, Ariel and {Groom}, Steven and {Hacopians}, Eugean and {Hale}, David and {Henning}, John and {Ho}, Anna Y.~Q. and {Hover}, David and {Howell}, Justin and {Hung}, Tiara and {Huppenkothen}, Daniela and {Imel}, David and {Ip}, Wing-Huen and {Ivezi{\'c}}, {\v{Z}}eljko and {Jackson}, Edward and {Jones}, Lynne and {Juric}, Mario and {Kasliwal}, Mansi M. and {Kaspi}, S. and {Kaye}, Stephen and {Kelley}, Michael S.~P. and {Kowalski}, Marek and {Kramer}, Emily and {Kupfer}, Thomas and {Landry}, Walter and {Laher}, Russ R. and {Lee}, Chien-De and {Lin}, Hsing Wen and {Lin}, Zhong-Yi and {Lunnan}, Ragnhild and {Giomi}, Matteo and {Mahabal}, Ashish and {Mao}, Peter and {Miller}, Adam A. and {Monkewitz}, Serge and {Murphy}, Patrick and {Ngeow}, Chow-Choong and {Nordin}, Jakob and {Nugent}, Peter and {Ofek}, Eran and {Patterson}, Maria T. and {Penprase}, Bryan and {Porter}, Michael and {Rauch}, Ludwig and {Rebbapragada}, Umaa and {Reiley}, Dan and {Rigault}, Mickael and {Rodriguez}, Hector and {van Roestel}, Jan and {Rusholme}, Ben and {van Santen}, Jakob and {Schulze}, S. and {Shupe}, David L. and {Singer}, Leo P. and {Soumagnac}, Maayane T. and {Stein}, Robert and {Surace}, Jason and {Sollerman}, Jesper and {Szkody}, Paula and {Taddia}, F. and {Terek}, Scott and {Van Sistine}, Angela and {van Velzen}, Sjoert and {Vestrand}, W. Thomas and {Walters}, Richard and {Ward}, Charlotte and {Ye}, Quan-Zhi and {Yu}, Po-Chieh and {Yan}, Lin and {Zolkower}, Jeffry},
        title = "{The Zwicky Transient Facility: System Overview, Performance, and First Results}",
      journal = {\pasp},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2019,
        month = jan,
       volume = {131},
       number = {995},
        pages = {018002},
          doi = {10.1088/1538-3873/aaecbe},
archivePrefix = {arXiv},
       eprint = {1902.01932},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019PASP..131a8002B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2016A&A...595A...1G,
       author = {{Gaia Collaboration} and {Prusti}, T. and {de Bruijne}, J.~H.~J. and
         {Brown}, A.~G.~A. and {Vallenari}, A. and {Babusiaux}, C. and
         {Bailer-Jones}, C.~A.~L. and {Bastian}, U. and {Biermann}, M. and
         {Evans}, D.~W. and {Eyer}, L. and {Jansen}, F. and {Jordi}, C. and
         {Klioner}, S.~A. and {Lammers}, U. and {Lindegren}, L. and {Luri}, X. and
         {Mignard}, F. and {Milligan}, D.~J. and {Panem}, C. and
         {Poinsignon}, V. and {Pourbaix}, D. and {Randich}, S. and {Sarri}, G. and
         {Sartoretti}, P. and {Siddiqui}, H.~I. and {Soubiran}, C. and
         {Valette}, V. and {van Leeuwen}, F. and {Walton}, N.~A. and
         {Aerts}, C. and {Arenou}, F. and {Cropper}, M. and {Drimmel}, R. and
         {H{\o}g}, E. and {Katz}, D. and {Lattanzi}, M.~G. and {O'Mullane}, W. and
         {Grebel}, E.~K. and {Holland}, A.~D. and {Huc}, C. and {Passot}, X. and
         {Bramante}, L. and {Cacciari}, C. and {Casta{\~n}eda}, J. and
         {Chaoul}, L. and {Cheek}, N. and {De Angeli}, F. and {Fabricius}, C. and
         {Guerra}, R. and {Hern{\'a}ndez}, J. and {Jean-Antoine-Piccolo}, A. and
         {Masana}, E. and {Messineo}, R. and {Mowlavi}, N. and
         {Nienartowicz}, K. and {Ord{\'o}{\~n}ez-Blanco}, D. and {Panuzzo}, P. and
         {Portell}, J. and {Richards}, P.~J. and {Riello}, M. and
         {Seabroke}, G.~M. and {Tanga}, P. and {Th{\'e}venin}, F. and
         {Torra}, J. and {Els}, S.~G. and {Gracia-Abril}, G. and
         {Comoretto}, G. and {Garcia-Reinaldos}, M. and {Lock}, T. and
         {Mercier}, E. and {Altmann}, M. and {Andrae}, R. and
         {Astraatmadja}, T.~L. and {Bellas-Velidis}, I. and {Benson}, K. and
         {Berthier}, J. and {Blomme}, R. and {Busso}, G. and {Carry}, B. and
         {Cellino}, A. and {Clementini}, G. and {Cowell}, S. and {Creevey}, O. and
         {Cuypers}, J. and {Davidson}, M. and {De Ridder}, J. and
         {de Torres}, A. and {Delchambre}, L. and {Dell'Oro}, A. and
         {Ducourant}, C. and {Fr{\'e}mat}, Y. and {Garc{\'\i}a-Torres}, M. and
         {Gosset}, E. and {Halbwachs}, J. -L. and {Hambly}, N.~C. and
         {Harrison}, D.~L. and {Hauser}, M. and {Hestroffer}, D. and
         {Hodgkin}, S.~T. and {Huckle}, H.~E. and {Hutton}, A. and
         {Jasniewicz}, G. and {Jordan}, S. and {Kontizas}, M. and {Korn}, A.~J. and
         {Lanzafame}, A.~C. and {Manteiga}, M. and {Moitinho}, A. and
         {Muinonen}, K. and {Osinde}, J. and {Pancino}, E. and {Pauwels}, T. and
         {Petit}, J. -M. and {Recio-Blanco}, A. and {Robin}, A.~C. and
         {Sarro}, L.~M. and {Siopis}, C. and {Smith}, M. and {Smith}, K.~W. and
         {Sozzetti}, A. and {Thuillot}, W. and {van Reeven}, W. and {Viala}, Y. and
         {Abbas}, U. and {Abreu Aramburu}, A. and {Accart}, S. and
         {Aguado}, J.~J. and {Allan}, P.~M. and {Allasia}, W. and
         {Altavilla}, G. and {{\'A}lvarez}, M.~A. and {Alves}, J. and
         {Anderson}, R.~I. and {Andrei}, A.~H. and {Anglada Varela}, E. and
         {Antiche}, E. and {Antoja}, T. and {Ant{\'o}n}, S. and {Arcay}, B. and
         {Atzei}, A. and {Ayache}, L. and {Bach}, N. and {Baker}, S.~G. and
         {Balaguer-N{\'u}{\~n}ez}, L. and {Barache}, C. and {Barata}, C. and
         {Barbier}, A. and {Barblan}, F. and {Baroni}, M. and
         {Barrado y Navascu{\'e}s}, D. and {Barros}, M. and {Barstow}, M.~A. and
         {Becciani}, U. and {Bellazzini}, M. and {Bellei}, G. and
         {Bello Garc{\'\i}a}, A. and {Belokurov}, V. and {Bendjoya}, P. and
         {Berihuete}, A. and {Bianchi}, L. and {Bienaym{\'e}}, O. and
         {Billebaud}, F. and {Blagorodnova}, N. and {Blanco-Cuaresma}, S. and
         {Boch}, T. and {Bombrun}, A. and {Borrachero}, R. and {Bouquillon}, S. and
         {Bourda}, G. and {Bouy}, H. and {Bragaglia}, A. and {Breddels}, M.~A. and
         {Brouillet}, N. and {Br{\"u}semeister}, T. and {Bucciarelli}, B. and
         {Budnik}, F. and {Burgess}, P. and {Burgon}, R. and {Burlacu}, A. and
         {Busonero}, D. and {Buzzi}, R. and {Caffau}, E. and {Cambras}, J. and
         {Campbell}, H. and {Cancelliere}, R. and {Cantat-Gaudin}, T. and
         {Carlucci}, T. and {Carrasco}, J.~M. and {Castellani}, M. and
         {Charlot}, P. and {Charnas}, J. and {Charvet}, P. and {Chassat}, F. and
         {Chiavassa}, A. and {Clotet}, M. and {Cocozza}, G. and
         {Collins}, R.~S. and {Collins}, P. and {Costigan}, G. and {Crifo}, F. and
         {Cross}, N.~J.~G. and {Crosta}, M. and {Crowley}, C. and {Dafonte}, C. and
         {Damerdji}, Y. and {Dapergolas}, A. and {David}, P. and {David}, M. and
         {De Cat}, P. and {de Felice}, F. and {de Laverny}, P. and
         {De Luise}, F. and {De March}, R. and {de Martino}, D. and
         {de Souza}, R. and {Debosscher}, J. and {del Pozo}, E. and {Delbo}, M. and
         {Delgado}, A. and {Delgado}, H.~E. and {di Marco}, F. and
         {Di Matteo}, P. and {Diakite}, S. and {Distefano}, E. and
         {Dolding}, C. and {Dos Anjos}, S. and {Drazinos}, P. and
         {Dur{\'a}n}, J. and {Dzigan}, Y. and {Ecale}, E. and {Edvardsson}, B. and
         {Enke}, H. and {Erdmann}, M. and {Escolar}, D. and {Espina}, M. and
         {Evans}, N.~W. and {Eynard Bontemps}, G. and {Fabre}, C. and
         {Fabrizio}, M. and {Faigler}, S. and {Falc{\~a}o}, A.~J. and
         {Farr{\`a}s Casas}, M. and {Faye}, F. and {Federici}, L. and
         {Fedorets}, G. and {Fern{\'a}ndez-Hern{\'a}ndez}, J. and
         {Fernique}, P. and {Fienga}, A. and {Figueras}, F. and {Filippi}, F. and
         {Findeisen}, K. and {Fonti}, A. and {Fouesneau}, M. and {Fraile}, E. and
         {Fraser}, M. and {Fuchs}, J. and {Furnell}, R. and {Gai}, M. and
         {Galleti}, S. and {Galluccio}, L. and {Garabato}, D. and
         {Garc{\'\i}a-Sedano}, F. and {Gar{\'e}}, P. and {Garofalo}, A. and
         {Garralda}, N. and {Gavras}, P. and {Gerssen}, J. and {Geyer}, R. and
         {Gilmore}, G. and {Girona}, S. and {Giuffrida}, G. and {Gomes}, M. and
         {Gonz{\'a}lez-Marcos}, A. and {Gonz{\'a}lez-N{\'u}{\~n}ez}, J. and
         {Gonz{\'a}lez-Vidal}, J.~J. and {Granvik}, M. and {Guerrier}, A. and
         {Guillout}, P. and {Guiraud}, J. and {G{\'u}rpide}, A. and
         {Guti{\'e}rrez-S{\'a}nchez}, R. and {Guy}, L.~P. and {Haigron}, R. and
         {Hatzidimitriou}, D. and {Haywood}, M. and {Heiter}, U. and
         {Helmi}, A. and {Hobbs}, D. and {Hofmann}, W. and {Holl}, B. and {Holland
        }, G. and {Hunt}, J.~A.~S. and {Hypki}, A. and {Icardi}, V. and
         {Irwin}, M. and {Jevardat de Fombelle}, G. and {Jofr{\'e}}, P. and
         {Jonker}, P.~G. and {Jorissen}, A. and {Julbe}, F. and
         {Karampelas}, A. and {Kochoska}, A. and {Kohley}, R. and
         {Kolenberg}, K. and {Kontizas}, E. and {Koposov}, S.~E. and
         {Kordopatis}, G. and {Koubsky}, P. and {Kowalczyk}, A. and
         {Krone-Martins}, A. and {Kudryashova}, M. and {Kull}, I. and
         {Bachchan}, R.~K. and {Lacoste-Seris}, F. and {Lanza}, A.~F. and
         {Lavigne}, J. -B. and {Le Poncin-Lafitte}, C. and {Lebreton}, Y. and
         {Lebzelter}, T. and {Leccia}, S. and {Leclerc}, N. and
         {Lecoeur-Taibi}, I. and {Lemaitre}, V. and {Lenhardt}, H. and
         {Leroux}, F. and {Liao}, S. and {Licata}, E. and
         {Lindstr{\o}m}, H.~E.~P. and {Lister}, T.~A. and {Livanou}, E. and
         {Lobel}, A. and {L{\"o}ffler}, W. and {L{\'o}pez}, M. and
         {Lopez-Lozano}, A. and {Lorenz}, D. and {Loureiro}, T. and
         {MacDonald}, I. and {Magalh{\~a}es Fernandes}, T. and {Managau}, S. and
         {Mann}, R.~G. and {Mantelet}, G. and {Marchal}, O. and
         {Marchant}, J.~M. and {Marconi}, M. and {Marie}, J. and {Marinoni}, S. and
         {Marrese}, P.~M. and {Marschalk{\'o}}, G. and {Marshall}, D.~J. and
         {Mart{\'\i}n-Fleitas}, J.~M. and {Martino}, M. and {Mary}, N. and
         {Matijevi{\v{c}}}, G. and {Mazeh}, T. and {McMillan}, P.~J. and
         {Messina}, S. and {Mestre}, A. and {Michalik}, D. and {Millar}, N.~R. and
         {Miranda}, B.~M.~H. and {Molina}, D. and {Molinaro}, R. and
         {Molinaro}, M. and {Moln{\'a}r}, L. and {Moniez}, M. and
         {Montegriffo}, P. and {Monteiro}, D. and {Mor}, R. and {Mora}, A. and
         {Morbidelli}, R. and {Morel}, T. and {Morgenthaler}, S. and
         {Morley}, T. and {Morris}, D. and {Mulone}, A.~F. and {Muraveva}, T. and
         {Musella}, I. and {Narbonne}, J. and {Nelemans}, G. and {Nicastro}, L. and
         {Noval}, L. and {Ord{\'e}novic}, C. and {Ordieres-Mer{\'e}}, J. and
         {Osborne}, P. and {Pagani}, C. and {Pagano}, I. and {Pailler}, F. and
         {Palacin}, H. and {Palaversa}, L. and {Parsons}, P. and {Paulsen}, T. and
         {Pecoraro}, M. and {Pedrosa}, R. and {Pentik{\"a}inen}, H. and
         {Pereira}, J. and {Pichon}, B. and {Piersimoni}, A.~M. and
         {Pineau}, F. -X. and {Plachy}, E. and {Plum}, G. and {Poujoulet}, E. and
         {Pr{\v{s}}a}, A. and {Pulone}, L. and {Ragaini}, S. and {Rago}, S. and
         {Rambaux}, N. and {Ramos-Lerate}, M. and {Ranalli}, P. and {Rauw}, G. and
         {Read}, A. and {Regibo}, S. and {Renk}, F. and {Reyl{\'e}}, C. and
         {Ribeiro}, R.~A. and {Rimoldini}, L. and {Ripepi}, V. and {Riva}, A. and
         {Rixon}, G. and {Roelens}, M. and {Romero-G{\'o}mez}, M. and
         {Rowell}, N. and {Royer}, F. and {Rudolph}, A. and {Ruiz-Dern}, L. and
         {Sadowski}, G. and {Sagrist{\`a} Sell{\'e}s}, T. and {Sahlmann}, J. and
         {Salgado}, J. and {Salguero}, E. and {Sarasso}, M. and {Savietto}, H. and
         {Schnorhk}, A. and {Schultheis}, M. and {Sciacca}, E. and {Segol}, M. and
         {Segovia}, J.~C. and {Segransan}, D. and {Serpell}, E. and
         {Shih}, I. -C. and {Smareglia}, R. and {Smart}, R.~L. and {Smith}, C. and
         {Solano}, E. and {Solitro}, F. and {Sordo}, R. and {Soria Nieto}, S. and
         {Souchay}, J. and {Spagna}, A. and {Spoto}, F. and {Stampa}, U. and
         {Steele}, I.~A. and {Steidelm{\"u}ller}, H. and {Stephenson}, C.~A. and
         {Stoev}, H. and {Suess}, F.~F. and {S{\"u}veges}, M. and {Surdej}, J. and
         {Szabados}, L. and {Szegedi-Elek}, E. and {Tapiador}, D. and
         {Taris}, F. and {Tauran}, G. and {Taylor}, M.~B. and {Teixeira}, R. and
         {Terrett}, D. and {Tingley}, B. and {Trager}, S.~C. and {Turon}, C. and
         {Ulla}, A. and {Utrilla}, E. and {Valentini}, G. and {van Elteren}, A. and
         {Van Hemelryck}, E. and {van Leeuwen}, M. and {Varadi}, M. and
         {Vecchiato}, A. and {Veljanoski}, J. and {Via}, T. and {Vicente}, D. and
         {Vogt}, S. and {Voss}, H. and {Votruba}, V. and {Voutsinas}, S. and
         {Walmsley}, G. and {Weiler}, M. and {Weingrill}, K. and {Werner}, D. and
         {Wevers}, T. and {Whitehead}, G. and {Wyrzykowski}, {\L}. and
         {Yoldas}, A. and {{\v{Z}}erjal}, M. and {Zucker}, S. and {Zurbach}, C. and
         {Zwitter}, T. and {Alecu}, A. and {Allen}, M. and {Allende Prieto}, C. and
         {Amorim}, A. and {Anglada-Escud{\'e}}, G. and {Arsenijevic}, V. and
         {Azaz}, S. and {Balm}, P. and {Beck}, M. and {Bernstein}, H. -H. and
         {Bigot}, L. and {Bijaoui}, A. and {Blasco}, C. and {Bonfigli}, M. and
         {Bono}, G. and {Boudreault}, S. and {Bressan}, A. and {Brown}, S. and
         {Brunet}, P. -M. and {Bunclark}, P. and {Buonanno}, R. and
         {Butkevich}, A.~G. and {Carret}, C. and {Carrion}, C. and {Chemin}, L. and
         {Ch{\'e}reau}, F. and {Corcione}, L. and {Darmigny}, E. and
         {de Boer}, K.~S. and {de Teodoro}, P. and {de Zeeuw}, P.~T. and
         {Delle Luche}, C. and {Domingues}, C.~D. and {Dubath}, P. and
         {Fodor}, F. and {Fr{\'e}zouls}, B. and {Fries}, A. and {Fustes}, D. and
         {Fyfe}, D. and {Gallardo}, E. and {Gallegos}, J. and {Gardiol}, D. and
         {Gebran}, M. and {Gomboc}, A. and {G{\'o}mez}, A. and {Grux}, E. and
         {Gueguen}, A. and {Heyrovsky}, A. and {Hoar}, J. and {Iannicola}, G. and
         {Isasi Parache}, Y. and {Janotto}, A. -M. and {Joliet}, E. and
         {Jonckheere}, A. and {Keil}, R. and {Kim}, D. -W. and {Klagyivik}, P. and
         {Klar}, J. and {Knude}, J. and {Kochukhov}, O. and {Kolka}, I. and
         {Kos}, J. and {Kutka}, A. and {Lainey}, V. and {LeBouquin}, D. and
         {Liu}, C. and {Loreggia}, D. and {Makarov}, V.~V. and
         {Marseille}, M.~G. and {Martayan}, C. and {Martinez-Rubi}, O. and
         {Massart}, B. and {Meynadier}, F. and {Mignot}, S. and {Munari}, U. and
         {Nguyen}, A. -T. and {Nordlander}, T. and {Ocvirk}, P. and
         {O'Flaherty}, K.~S. and {Olias Sanz}, A. and {Ortiz}, P. and
         {Osorio}, J. and {Oszkiewicz}, D. and {Ouzounis}, A. and {Palmer}, M. and
         {Park}, P. and {Pasquato}, E. and {Peltzer}, C. and {Peralta}, J. and
         {P{\'e}turaud}, F. and {Pieniluoma}, T. and {Pigozzi}, E. and
         {Poels}, J. and {Prat}, G. and {Prod'homme}, T. and {Raison}, F. and
         {Rebordao}, J.~M. and {Risquez}, D. and {Rocca-Volmerange}, B. and
         {Rosen}, S. and {Ruiz-Fuertes}, M.~I. and {Russo}, F. and {Sembay}, S. and
         {Serraller Vizcaino}, I. and {Short}, A. and {Siebert}, A. and
         {Silva}, H. and {Sinachopoulos}, D. and {Slezak}, E. and {Soffel}, M. and
         {Sosnowska}, D. and {Strai{\v{z}}ys}, V. and {ter Linden}, M. and
         {Terrell}, D. and {Theil}, S. and {Tiede}, C. and {Troisi}, L. and
         {Tsalmantza}, P. and {Tur}, D. and {Vaccari}, M. and {Vachier}, F. and
         {Valles}, P. and {Van Hamme}, W. and {Veltz}, L. and {Virtanen}, J. and
         {Wallut}, J. -M. and {Wichmann}, R. and {Wilkinson}, M.~I. and
         {Ziaeepour}, H. and {Zschocke}, S.},
        title = "{The Gaia mission}",
      journal = {\aap},
     keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2016",
        month = "Nov",
       volume = {595},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201629272},
archivePrefix = {arXiv},
       eprint = {1609.04153},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...595A...1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2009Ap&SS.320..261C,
       author = {{Catelan}, M.},
        title = "{Horizontal branch stars: the interplay between observations and theory, and insights into the formation of the Galaxy}",
      journal = {\apss},
     keywords = {Galaxies: Local Group, Galaxy: formation, Galaxy: globular cluster: general, Stars: evolution, Stars: Hertzsprung-Russell diagram, Stars: horizontal-branch, Stars: variables: other, Astrophysics},
         year = 2009,
        month = apr,
       volume = {320},
        pages = {261-309},
          doi = {10.1007/s10509-009-9987-8},
archivePrefix = {arXiv},
       eprint = {astro-ph/0507464},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009Ap&SS.320..261C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{1939Obs....62..104O,
       author = {{Oosterhoff}, P.~T.},
        title = "{Some remarks on the variable stars in globular clusters}",
      journal = {The Observatory},
         year = 1939,
        month = apr,
       volume = {62},
        pages = {104-109},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1939Obs....62..104O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@Misc{scipy,
  author =    {Eric Jones and Travis Oliphant and Pearu Peterson and others},
  title =     {{SciPy}: Open source scientific tools for {Python}},
  year =      {2001},
  url = "http://www.scipy.org/"
}




@book{python,
 author = {Van Rossum, Guido and Drake, Fred L.},
 title = {Python 3 Reference Manual},
 year = {2009},
 isbn = {1441412697},
 publisher = {CreateSpace},
 address = {Scotts Valley, CA}
}



@article{numpy,
   author = "{van~der~Walt}, Stefan  and Colbert, S. Chris and Varoquaux, Gael",
   title = "The NumPy Array: A Structure for Efficient Numerical Computation",
   journal = "Computing in Science \& Engineering",
   year = "2011",
   volume = "13",
   number = "2", 
   pages = "22-30",
   url = "http://scitation.aip.org/content/aip/journal/cise/13/2/10.1109/MCSE.2011.37",
   doi = "http://dx.doi.org/10.1109/MCSE.2011.37" 
}


@article{matplotlib,
   author = "Hunter, John D.",
   title = "Matplotlib: A 2D Graphics Environment",
   journal = "Computing in Science \& Engineering",
   year = "2007",
   volume = "9",
   number = "3", 
   pages = "90-95",
   url = "http://scitation.aip.org/content/aip/journal/cise/9/3/10.1109/MCSE.2007.55",
   doi = "http://dx.doi.org/10.1109/MCSE.2007.55" 
}


@misc{seaborn,
  author       = {Michael Waskom and Olga Botvinnik and drewokane and Paul Hobson and Yaroslav Halchenko and Saulius Lukauskas and Jordi Warmenhoven and John B. Cole and Stephan Hoyer and Jake Vanderplas and gkunter and Santi Villalba and Eric Quintero and Marcel Martin and Alistair Miles and Kyle Meyer and Tom Augspurger and Tal Yarkoni and Pete Bachant and Constantine Evans and Clark Fitzgerald and Tamas Nagy and Erik Ziegler and Tobias Megies and Daniel Wehner and Samuel St-Jean and Luis Pedro Coelho and Gregory Hitz and Antony Lee and Luc Rocher},
  title        = {seaborn: v0.7.0 (January 2016)},
  month        = jan,
  year         = 2016,
  doi          = {10.5281/zenodo.45133},
  url          = {http://dx.doi.org/10.5281/zenodo.45133}
}


@misc{pandas,
author = {Mckinney, Wes},
month = jan,
year = {2010},
pages     = { 56 - 61 },
title = {Data Structures for Statistical Computing in Python},
booktitle = {Proceedings of the 9th Python in Science Conference},
editor    = { {S}t\'efan van der {W}alt and {J}arrod {M}illman },
doi       = { 10.25080/Majora-92bf1922-00a }
}





@ARTICLE{astropy,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and 
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and 
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and 
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and 
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and 
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and 
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and 
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and 
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and 
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and 
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and 
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and 
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@INPROCEEDINGS{Koposov2006,
       author = {{Koposov}, S. and {Bartunov}, O.},
        title = "{Q3C, Quad Tree Cube -- The new Sky-indexing Concept for Huge Astronomical Catalogues and its Realization for Main Astronomical Queries (Cone Search and Xmatch) in Open Source Database PostgreSQL}",
    booktitle = {Astronomical Data Analysis Software and Systems XV},
         year = 2006,
       editor = {{Gabriel}, C. and {Arviset}, C. and {Ponz}, D. and {Enrique}, S.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {351},
        month = jul,
        pages = {735},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..735K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1996AJ....112.1487H,
       author = {{Harris}, William E.},
        title = "{A Catalog of Parameters for Globular Clusters in the Milky Way}",
      journal = {\aj},
     keywords = {GLOBULAR CLUSTERS: GENERAL, CATALOGS},
         year = 1996,
        month = oct,
       volume = {112},
        pages = {1487},
          doi = {10.1086/118116},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996AJ....112.1487H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2010arXiv1012.3224H,
       author = {{Harris}, William E.},
        title = "{A New Catalog of Globular Clusters in the Milky Way}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = dec,
          eid = {arXiv:1012.3224},
        pages = {arXiv:1012.3224},
archivePrefix = {arXiv},
       eprint = {1012.3224},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010arXiv1012.3224H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


